BROJA-2PID: A robust estimator for bivariate partial information decomposition

Makkeh, Theis, and Vicente found in [8] that Cone Programming model is the most robust to compute the Bertschinger et al. partial information decompostion (BROJA PID) measure [1]. We developed a production-quality robust software that computes the BROJA PID measure based on the Cone Programming model. In this paper, we prove the important property of strong duality for the Cone Program and prove an equivalence between the Cone Program and the original Convex problem. Then describe in detail our software and how to use it.\newline\indent

==> figures/implementation.tex <==
We implemented the exponential cone program~\eqref{eq:BROJA-ExpCone} into Python and used a conic optimization solver to get the desired solution. Note that we are aware of only two Conic Optimization software toolboxes which allow to solve exponential cone programs, ECOS and SCS. The current version of \textsc{Broja\_2pid} utilities ECOS to solve the exponential cone program. ECOS\footnote{We use the version from Nov~8, 2016.} is a lightweight numerical software for solving convex cone programs~\cite{Domahidi-Chu-Boyd:ECOS:13}. 

This section describes the \textsc{Broja\_2pid} package form the user's perspective.  We will explain the framework of \textsc{Broja\_2pid} and its functions. Then we describe the input and tuning parameters. Finally, we will discuss the output.
%
%
\subsection{Computing Bivariate PID}
	In this subsection, we will explain how \textsc{Broja\_2pid} works. Figure~\ref{fig:and-gate} is an example of using \textsc{Broja\_2pid} package to compute the partial information decomposition of the \textsc{And} distribution, $X = Y\operatorname{AND}Z$ where $Y$ and $Z$ are independent and uniformly distributed in $\{0,1\}$.
%	\begin{wrapfigure}[24]{r}{0.5\textwidth}
%	  \scalebox{0.65}[0.65]{
%	  		\pythonexternal{test_and_gate.py}
%	  	}
%	    \caption{Computing the bivariate PID of the \textsc{And} gate using \textsc{Broja\_2pid}.} \label{fig:and-gate}
%	\end{wrapfigure}
	\begin{figure}[H]
		\centering
		\scalebox{0.7}[0.7]{
			\pythonexternal{test_and_gate.py}
			}
		\caption{Computing the partial information decomposition of the \textsc{And} gate using \textsc{Broja\_2pid}.} \label{fig:and-gate}
	\end{figure} 
	
	We will go through out the example, Figure~\ref{fig:and-gate}, to explain how \textsc{Broja\_2pid} works. The main function in \textsc{Broja\_2pid} package is\pythoninline{pid()}. It is a wrap up function which is used to compute the partial information decomposition. First,\pythoninline{pid()} prepares the ``ingredients'' of~\eqref{eq:BROJA-ExpCone}. Then it calls the conic optimization solver to find the optimal solution of~\eqref{eq:BROJA-ExpCone}. Finally, it receives from the conic optimization solver the required solution to compute the decomposition. 
	
	The ``ingredients'' of~\eqref{eq:BROJA-ExpCone} are the marginal and coupling equations, generalized inequalities, and the objective function. So,\pythoninline{pid()} needs to compute and store $b^\y_{x,y}$ and $b^\z_{x,z}$, the marginal distributions of $(X,Y)$ and $(X,Z)$. For this,\pythoninline{pid()} requires a distribution of $X,Y,$ and $Z$. In Figure~\ref{fig:and-gate}, the distribution comes from the \textsc{And} gate. 
	
	The distribution must always be defined as a mapping (Python dictionary) of $(x,y,z)$, \textit{triplet}, to its respective probability, \textit{number}. E.g., $(0,0,0)$ occurs with probability $\nicefrac{1}{4}$ from the \textsc{And} distribution. So the \textsc{And} distribution is defined as a Python dictionary,\pythoninline{andgate=dict()} where\pythoninline{andgate[ (0,0,0) ]=.25} is assigning the key ``$(0,0,0)$'' a value ``0.25''.
	
	Note that the user doesn't have to add the triplets with zero probability to the dictionary since\pythoninline{pid()} will always discard such triplets. In~\cite{makkeh-theis-vicente:pidOpt:2017}, the authors discussed in details how to handle the triplets with zero probability. The input of\pythoninline{pid()} is explained in details in the following subsection.
	
	Now we briefly describe how\pythoninline{pid()} proceeds to return the promised decomposition. \pythoninline{pid()} calls the conic optimization solver and provides it with the ``ingredients'' of~\eqref{eq:BROJA-ExpCone} as a part of the solver's input. The solver finds the optimal solution of~\eqref{eq:BROJA-ExpCone} and~\eqref{eq:BROJA-DExpCone}. When the solver halts it returns the primal and dual solutions. Using the returned solution, \pythoninline{pid()} computes the decomposition based on equation~\eqref{eq:bpid-4}.  The full process is explained in Figure~\ref{fig:flow-chart}.
	
	Finally,\pythoninline{pid()} returns a Python dictionary, \pythoninline{returndata} containing the partial information decomposition and data about the quality of the conic optimization solver's solution. In Subsection~\ref{subsec:output} we give a detailed explanation on how to compute the quality's data and Table~\ref{tab:output} contains a description of the keys and values of \pythoninline{returndata}.

	E.g., in the returned dictionary\pythoninline{returndata} for the \textsc{And} gate,\pythoninline{returndict['CI']} contains the quantity of synergistic information and\pythoninline{returndict['Num_err'][0]} the maximum primal feasibility violation of~\eqref{eq:BROJA-ExpCone}. 
	
	Note that conic optimization solver is always supposed to return a solution. So, \textsc{Broja\_2pid} will raise an exception,\pythoninline{BROJA\_2PID\_Exception}, when no solution is returned. 
%	
%
%		The conic optimization solver halts returning a list of lists $w$ containing the primal solution where $w_{x,y,z} = (r_{x,y,z}, p_{x,y,z}, q_{x,y,z})$, an list of lists $\eta$ where $\eta_{xyz}= (\lambda_{x,y},\lambda_{x,z}, \mu_{x,y,z})$ as the dual of equations in~\eqref{eq:BROJA-ExpCone}, and a list $\theta$ where $\theta_{x,y,z} = \nu_{x,y,z}$ as the dual of generalized inequalities in~\eqref{eq:BROJA-ExpCone}.
%	 
%		Now \pythoninline{pid()} has the optimal solutions of~\eqref{eq:BROJA-ExpCone} and~\eqref{eq:BROJA-DExpCone} stored in $w,\eta,$ and $\theta$. From $w$, \pythoninline{pid()} takes $q$ and discard all $q_{x,y,z} = 0$ and uses the refined $q$ to compute $SI(X;Y,Z), CI(X;Y,Z), UI(X;Y\backslash Z),$ and  $UI(X;Z\backslash Y)$. Also it uses $w,\eta,$ and $\theta$ with no modifications to compute the optimality guarantees,  primal, dual feasibility, and duality gap. 

%	
	\begin{figure}
		\centering
		\includegraphics[height=8cm, width=15cm]{flow_chart_2.png}
		\caption{\textsc{Broja\_2pid} workflow. Left is the flow in \texttt{pid()}. Right is the flow in ECOS. The arrows with oval tail indicate passing of data whereas the ones with line tail indicate time flow.}
		\label{fig:flow-chart}
	\end{figure}     
%
%			   
\subsection{Input and Parameters}\label{subsec:input}
	In \textsc{Broja\_2pid} package,\pythoninline{pid()} is the function which the user needs to compute the partial information decomposition. The function\pythoninline{pid()} takes as input a Python dictionary.
	
	The Python dictionary will represent a probability distribution. This distribution computes the vectors $b^\y_{x,y}$ and $b^\z_{x,z}$ for the  the marginal equations in \eqref{eq:BROJA-ExpCone}. A key of the Python dictionary is a \textit{triplet} of $(x,y,z)$ which is a possible outcome of the random variables $X,Y,$ and~$Z$. A value of the key~$(x,y,z)$ in the Python dictionary is a \textit{number} which is the probability of $X=x,Y=y,$ and $Z=z$. 
	\paragraph{Solver parameters.} The conic optimization solver has to make sure while seeking the optimal solution of~\eqref{eq:BROJA-ExpCone} that $w$ and $(\eta, \theta)$ are feasible and (ideally) should halt when the duality gap is zero, i.e., $w$ and $(\eta, \theta)$ are optimal. But  $w$ and $(\eta, \theta)$ entries belong to $\RR$ and computers represent real numbers up to floating precisions. So the conic optimization solver consider a solution feasible, none of the constraints are violated, or optimal, duality gap is zero, up to a numerical precision (tolerance). The conic optimization solver allows the user to modify the feasibility and optimality tolerances along with couple other parameters which are described in Table~\ref{tab:ecos}. 
%			\begin{equation*}
%				\begin{split}
%					\frac{Ax - b}{\max(1,\norm{b})}						&\le \epsilon_1\\
%					\frac{Gx - h + s}{\max(1,\norm{h})}					&\le \epsilon_2\\
%					\frac{A^T\lambda + G^T\mu + c}{\max(1,\norm{c})}	&\le \epsilon_3\\
%					c^Tx + b^T\lambda + h^T\mu							&\le \epsilon_4,
%				\end{split}
%			\end{equation*}
%			where $\epsilon_1,\epsilon_2,\epsilon_3,\epsilon_4$ are the numerical precision or tolerance, $s\le_K 0$, and $\norm{\cdot}$ is the 2-norm unless specified. .  ``ECOS'' which \pythoninline{pid()} uses to solve~\eqref{eq:BROJA-ExpCone} has allowed the user to choose such $\epsilon$'s and other parameters which tune the final solution. ``ECOS'' parameters are the following
	\begin{table}[H]
		\centering
		\scalebox{0.9}[0.9]{
		\begin{tabular}{ll}
		\toprule
		Parameter 				& Description 												\\
		\midrule
		\texttt{feastol}		& 	primal/dual feasibility tolerance 						\\
		\texttt{abstol}			&	absolute tolerance on duality gap						\\
		\texttt{reltol}			&	relative tolerance on duality gap						\\
		\texttt{feastol\_inacc} &	primal/dual infeasibility \textit{relaxed} tolerance	\\
		\texttt{abstol\_inacc}	&	absolute \textit{relaxed} tolerance on duality gap		\\
		\texttt{reltol\_inacc}	&	\textit{relaxed} relative duality gap					\\	
		\texttt{max\_iter}		&	maximum number of iterations that ``ECOS'' does			\\ 
		\bottomrule
		\end{tabular}%
		}%
		\caption[Parameters (tolerances) of ECOS]{Parameters (tolerances) of ECOS\footnotemark.}\label{tab:ecos}
	\end{table}
	\footnotetext{For more explanation see~\url{https://github.com/embotech/ecos}.}
	
		\begin{wrapfigure}[7]{r}{0.5\textwidth}
			\centering
		  	\pythonexternal{test_parameters.py}
		    \caption{Tuning parameters} \label{fig:tune}
		\end{wrapfigure}
	In order to change the default conic optimization solver parameters, the user should pass them to\pythoninline{pid()} as a dictionary. E.g.~in Figure~\ref{fig:tune}, we change the maximum number of iterations which the solver can do. For this we created a dictionary,\pythoninline{parms=dict()}. Then we set a desired value,\pythoninline{1000}, for the key\pythoninline{'max_iter'}. Finally, we are required to pass\pythoninline{parms} to\pythoninline{pid()} as a dictionary,\pythoninline{pid(andgate,**parms)}. Note in the defined dictionary\pythoninline{parms}, the user only need to define the keys which the user wants to change their values.
	
	There is another type of parameters, namely,\pythoninline{output} which is an integer in~$\{0,1,2\}$. It is a parameter which determines the printing mode of\pythoninline{pid()}. Meaning that it allows the user to control what will be printed on the screen. Table~\ref{tab:printing-mode} gives a detailed description of the printing mode.
		\begin{table}[H]
			\centering
			\scalebox{0.9}[0.9]{
			\begin{tabular}{ll}
				\toprule
				\texttt{output}	& Description 																	\\
				\midrule
				0 (default)		& \pythoninline{pid()} prints its output (python dictionary, see Subsection~\ref{subsec:output}).						\\
				1				& In addition to\pythoninline{output= 0}, \pythoninline{pid()} prints a flags when it starts preparing~\eqref{eq:BROJA-ExpCone}\\
			     				& and another flag when it calls the conic optimization solver.															\\
				2				& In addition to\pythoninline{output= 1}, \pythoninline{pid()} prints the conic optimization solver's output\footnotemark.	\\
				\bottomrule
			\end{tabular}%
			}%
			\caption{Description of the printing mode in \texttt{pid()}.}\label{tab:printing-mode}
		\end{table}
		\footnotetext{The conic optimization solver usually prints out the problem statistics and the status of optimization.}

\subsection{Returned Data}\label{subsec:output}
	The function\pythoninline{pid()} returns a Python dictionary called\pythoninline{returndata}. Table~\ref{tab:output} describes the returned dictionary.
	\begin{table}[H]
		\centering
		\scalebox{1}[1]{
		\begin{tabular}{ll}
		\toprule
		Key 							& Value 																	\\
		\midrule
		\pythoninline{'SI'}				& Shared information, $\SI(X;Y,Z)$.											\\
		\pythoninline{'UIY'}			& Unique information of $Y$, $\UI(X;Y\backslash Z)$. 						\\
		\pythoninline{'UIZ'}			& Unique information of $Z$, $\UI(X;Z\backslash Y)$.						\\
		\pythoninline{'CI'} 			& Synergistic information, $\CI(X;Y,Z)$.									\\
		\pythoninline{'Num_err'}		& information about the quality of the solution. 							\\
		\pythoninline{'Solver'}			& name of the solver used to optimize~\eqref{eq:the-BROJA-CP}\footnotemark.	\\ 
		\bottomrule
		\end{tabular}%
		} %
		\caption{Description of {\ttm returndata}, the Python dictionary returned by \texttt{pid()}.}\label{tab:output}
	\end{table}
	\footnotetext{In this version we are only using ECOS, but other solvers might be added in the future.}
	Let $w,\eta,$ and $\theta$ be the lists returned by the conic optimization solver where $w_{x,y,z} = [r_{x,y,z},p_{x,y,z},q_{x,y,z}],$ $\eta_{x,y,z}= [\lambda_{x,y},\lambda_{x,z}, \mu_{x,y,z}],$ and $\theta_{x,y,z} = [\nu_{x,y,z}]$. Note that $w$ is the primal solution and $(\eta,\theta)$ is the dual solution. The dictionary\pythoninline{returndata} gives the user access to the partial information decomposition, namely, shared, unique, and synergistic information. The partial information decomposition is computed using only the positive values $q_{x,y,z}$. The value of\pythoninline{returndata['Num_err']} is a triplet such that the primal feasibility violation is\pythoninline{returndata['Num_err'][0]}, the dual feasibility violation is \pythoninline{returndata['Num_err'][1]}, and\pythoninline{returndata['Num_err'][2]} is the duality gap violation. In what follows we will explain how we compute the violations of primal and dual feasibility in addition to that of duality gap. 
	
	The primal feasibility of~\eqref{eq:BROJA-ExpCone} is
	\begin{equation}\label{eq:primal-feas}
		\begin{split}
			q_{x,y,*} = b^\y_{x,y}\\
			q_{x,*,z} = b^\z_{x,z}\\
			q_{*,y,z} = p_{x,y,z}\\
			(-r_{x,y,z},-p_{x,y,z},-q_{x,y,z}) &\le_{\mathcal K_{\exp}} 0
		\end{split}
	\end{equation}
	We check the violation of $q_{x,y,z}\ge 0$ which is required by the $\mathcal K_{\exp}$. Since all the non-positive $q_{x,y,z}$ are discarded when computing the decomposition, we check if the marginal equations are violated using only the positive $q_{x,y,z}$. The coupling equations are ignored since they are just assigning values to the $p_{x,y,z}$ variables. So,\pythoninline{returndata['Num_err'][0]} (primal feasibility violation) is computed using the following 
	\begin{equation*}
		\begin{split}
			q'_{x,y,z} &=\begin{cases}
				0 &~\text{if $q_{x,y,z} \le 0$}\\
				q_{x,y,z} &~\text{otherwise}
			\end{cases}\\
			\delta &=\max_{x,y,z}( \abs{q'_{x,y,*} - b^\y_{x,y}}, \abs{q'_{x,*,z} - b^\z_{x,z}}, -q_{x,y,z})
		\end{split}
	\end{equation*} 
	The dual feasibility of~\eqref{eq:BROJA-DExpCone} is
	\begin{equation}\label{eq:daul-feas}
		\lambda_{x,y}	+	\lambda_{x,z}	+	\mu_{*,y,z}	+ 1	+	\ln(-\mu_{x,y,z}) \ge 0
	\end{equation}
	For dual feasibility violation, we check non negativity of~\eqref{eq:daul-feas};\pythoninline{returndata['Num_err'][1]} is equal to 
	\begin{equation*}
		\min_{x,y,z}(\lambda_{x,y}+\lambda_{x,z}+\mu_{*,y,z}+1+\ln(-\mu_{x,y,z}), 0)
	\end{equation*}
	When $w$ is the optimal solution of~\eqref{eq:BROJA-ExpCone}, we have 
	\begin{equation*}
	-\sum_{x,y,z} r_{x,y,z} = \sum_{x,y,z} q_{x,y,z}\log\frac{q_{x,y,z}}{q_{*,y,z}} = -H(X\mid Y,Z).
	\end{equation*}
	The duality gap of~\eqref{eq:BROJA-ExpCone} and~\eqref{eq:BROJA-DExpCone} is 
	\begin{equation}\label{eq:d-gap}
		-H(X\mid Y,Z) + \lambda^Tb,
	\end{equation}
	where%
	\begin{equation*}	 
			\lambda^Tb =\sum_{x,y}\lambda_{x,y}b^\y_{x,y} +\sum_{x,z}\lambda_{x,z}b^\z_{x,z}.
	\end{equation*}
	Since weak duality implies $H(X\mid Y,Z)\le \lambda^Tb$, so we are left to check the non negativity of~\eqref{eq:d-gap} to inspect the duality gap;\pythoninline{returndata['Num_err'][2]} is given by,%
	\begin{equation*}
			\max(-H(X\mid Y,Z) + \lambda^Tb,0)
	\end{equation*}

==> fragments.tex <==
be the target signals about a source signal $X$ in a complex system. E.g., two neurons $Y$ and $Z$ are excited by a stimulus $X$. Studying the responses of the neurons and their dependencies to characterize the relation of the responses to the stimulus is called \textit{neural coding}. In this case, a neurologist wants to investigate whether redundant information about $X$ is provided by both $Y$ and $Z$ or they behave synergistically. Also it is useful to figure out whether any of the targets provides unique information about $X$, i.e.~information that can be obtained only from that specific target. Thus, in such system we can differentiate between three quantities of information, shared, unique, and synergistic. $\SI(X;Y,Z)$ is the quantity of shared information which both $Y$ and $Z$ hold about $X$ that can be retrieved by looking at any of $Y$ and $Z$ alone. $\UI(X;Y\backslash Z)$ is the quantity of unique information which only $Y$ holds about $X$. Similarly, $\UI(X;Z\backslash Y)$, quantifies what $Z$ uniquely holds about $X$. $\CI(X;Y,Z)$ is the quantity of synergistic information about $X$ which can only be retrieved by knowing both $Y$ and $Z$. The mutual information $\MI(X;Y,Z)$ quantifies the overall information that $(Y,Z)$ has about $X$. So $\MI(X;Y,Z)$ is decomposed as follows
\begin{equation}\label{eq:MI-1}
	\MI(X;Y,Z) = \SI(X;Y,Z) + \UI(X;Y\backslash Z) + \UI(X;Z\backslash Y) + \CI(X;Y,Z)
\end{equation}
and $\SI(X;Y,Z)$ satisfy the following two equalities,
\begin{equation}\label{eq:MI-2}
\begin{split}
	\MI(X;Y) &= \SI(X;Y,Z) + \UI(X;Y\backslash Z)\\
	\MI(X;Z) &= \SI(X;Y,Z) + \UI(X;Z\backslash Y)
\end{split}
\end{equation}
Co-information, the negative interaction information defined in~\cite{mcgill1954multivariate}, is the difference between the information $Y$ and $X$ share when $Z$ is random and when $Z$ is determined,
\begin{equation*}
 	\CoI(X;Y,Z) := \MI(X;Y) - \MI(X;Y\mid Z)
\end{equation*}
using the chain rule of mutual information we get, 
\begin{equation}\label{eq:MI-3}
	\CoI(X;Y,Z) = \SI(X;Y,Z) - \CI(X;Y,Z)
\end{equation}
Finding the quantities $\SI(X;Y,Z), \CI(X;Y,Z), \UI(X;Y\backslash Z),$ and $\UI(X;Z\backslash Y)$ is called the partial information decomposition. From equations~\eqref{eq:MI-1}, \eqref{eq:MI-2}, and~\eqref{eq:MI-3} it suffices to find one of the quantities to get a partial information decomposition. The above problem, neural coding, and others have motivated scientists to seek a definition for the partial information decomposition. There are several definitions of the decomposition, none of which is considered the best. In this paper, we compute the Bertschinger et al.~\cite{bertschinger-rauh-olbrich-jost-ay:quantify:2014} partial information decomposition. Based on an operational interpretation of a decision problem, they defined $\UI(X; Y\backslash Z)$ as the minimum information that $Y$ holds on $X$ given the marginal distributions of $(X,Y)$ and $(X,Z)$.

Denote by $X$ the range of the random variable~$\mathbf{X}$, by $Y$ the range of~$\mathbf{Y}$, and by $Z$ the range of~$\mathbf{Z}$.  Further, let
\begin{align*}
	b^\y_{x,y} &:= \Prb\bigl( \mathbf{X} = x \land \mathbf{Y} = y \bigr) && \text{for all $x\in X$, $y\in Y$}\\
	b^\z_{x,z} &:= \Prb\bigl( \mathbf{X} = x \land \mathbf{Z} = z \bigr) && \text{for all $x\in X$, $y\in Y$}
\end{align*}
be the $(X,Y)$ and $(X,Z)$ marginals respectively. Bertschinger et al.~in~\cite{bertschinger-rauh-olbrich-jost-ay:quantify:2014} proved that solving any of the following optimization will yield the partial information decomposition. 
\begin{subequations}
	\begin{align}
		\UI(X;Y\backslash Z)	&=\min_{(x,y,z)\sim q}\MI(X;Y\mid Z)\label{eq:bpid-1}\\
		\UI(X;Z\backslash Y)	&=\min_{(x,y,z)\sim q}\MI(X;Z\mid Y)\label{eq:bpid-2}\\
		\SI(X;Y,Z)				&=\max_{(x,y,z)\sim q}\CoI(X;Y,Z)\label{eq:bpid-3}\\
		\CI(X;Y,Z)				&=\MI(X;Y,Z) - \min_{(x,y,z)\sim q}\MI(X;Y,Z).\label{eq:bpid-4}
	\end{align}
\end{subequations}
where $(x,y,z)\sim q$ stands for $(x,y,z)$ is distributed according to the probability distribution~$q$. The minimum ranges over all probability distributions $q \in [0,1]^{X\times Y\times Z}$ which satisfy the marginal equations
\begin{align*}
	q_{x,y,*} &= b^\y_{x,y}        &&\text{ for all $(x,y)\in X\times Y$}\\
	q_{x,*,z} &= b^\z_{x,z}        &&\text{ for all $(x,z)\in X\times Z$.}
\end{align*}
We use the notational convention that an asterisk ``$*$'' is to be read as ``sum over everything that can be plugged in here'';  e.g.,
\begin{equation*}
	q_{x,y,*} := \sum_{w} q_{x,y,w}.
\end{equation*}
(We don't use the symbol~$*$ in any other context.) Since all the optimizations~\eqref{eq:bpid-1},~\eqref{eq:bpid-2},\eqref{eq:bpid-3}, and~\eqref{eq:bpid-4}  are equivalent,~\cite[Lemma 4]{bertschinger-rauh-olbrich-jost-ay:quantify:2014}, we chose to optimize~\eqref{eq:bpid-4}. So, the goal is to minimize,
\begin{equation*}
	\MI_{(x,y,z)\sim q}(x;y,z ) = H_{(x,y,z)\sim q}(x) - H_{(x,y,z)\sim q}(x\mid y,z).
\end{equation*}

Since the distribution of~$x$ is fixed by the marginal equations, the first term in the sum is a constant, and we are left with minimizing negative conditional entropy,
\begin{equation*}
	-H(X\mid Y,Z)=\sum_{x,y,z} q_{x,y,z}\log\frac{q_{x,y,z}}{q_{*,y,z}}
\end{equation*}
The conditional entropy is computed in bits and so minimizing $\sum_{x,y,z} q_{x,y,z}\ln(\nicefrac{q_{x,y,z}}{q_{*,y,z}})$ and multiplying the result by $\log(2)$ returns the optimal negative conditional entropy. So, the convex optimization problem in~\cite{bertschinger-rauh-olbrich-jost-ay:quantify:2014} is the following:
\begin{equation}\label{eq:the-BROJA-CP}\tag{\mbox{CP}}
	\begin{aligned}
		\text{minimize }         &\sum_{x,y,z} q_{x,y,z}\ln\frac{q_{x,y,z}}{q_{*,y,z}}  &&\text{ over $q\in\RR^{X\times Y\times Z}$}\\
		\text{subject to }\quad  & q_{x,y,*} = b^\y_{x,y}        &&\text{ for all $(x,y)\in X\times Y$}\\
		{}                       & q_{x,*,z} = b^\z_{x,z}        &&\text{ for all $(x,z)\in X\times Z$}\\
		{}                       & q_{x,y,z} \ge 0               &&\text{ for all $(x,y,z)\in X\times Y\times Z$}\\
	\end{aligned}
\end{equation}
Bertschinger et al.~\cite{bertschinger-rauh-olbrich-jost-ay:quantify:2014}, while optimizing~\eqref{eq:the-BROJA-CP} found that either the computations can give wrong results or takes immensely long to converge. Makkeh, Theis, and Vicente in~\cite{makkeh-theis-vicente:pidOpt:2017} have studied the solution of~\eqref{eq:the-BROJA-CP} and formulated~\eqref{eq:the-BROJA-CP} as an exponential cone program~\eqref{eq:BROJA-ExpCone} which will be explained in Section ~\ref{sec:expcone}. The conic optimization~\eqref{eq:BROJA-ExpCone} can be solved efficiently and gives sufficiently correct decomposition.

We implemented a solver, \textsc{Broja\_2pid}, in Python that solves the conic optimization problem~\eqref{eq:BROJA-ExpCone} and thus finding the partial information decomposition defined by Bertschinger et al. The hardcore of \textsc{Broja\_2pid} is finding the optimal solution of a cone program. So in the next section we will explain conic optimization in a nutshell, briefly discuss its convergence to optimal solution, and then explain the formulation of~\eqref{eq:the-BROJA-CP} as a conic optimization problem. Section~\ref{sec:imp} we go through an example to describe how to use \textsc{Broja\_2pid} and explain the functions of \textsc{Broja\_2pid} package with their respective inputs and outputs. In Section~\ref{sec:case-study}, we close up by a case study of the \textsc{Broja\_2pid} against a group of instances and analyze the quality of the solution and running time. 

%William and Beer in~\cite{williams2010nonnegative} were the first to define a decomposition of mutual information into nonnegative quantities via the framework of \textit{partial information lattice}. They proposed the minimum information that either $Y$ and $Z$ can obtain about each outcome of $X$, averaged over all the possible outcomes, to be the shared information, $\SI(X;Y,Z).$ Unlike their framework this proposed measure couldn't give reliable values even for the \textsc{Xor} gate see~\cite{bertschinger2013shared}. Following this, Griffen et al.~\cite{griffith2014quantifying} defined synergy as the complement of information which $\MI(X;Y,Z)$ have given the marginal distributions of $(X,Y)$ and $(X,Z)$. Bertschinger et al.~in~\cite{bertschinger-rauh-olbrich-jost-ay:quantify:2014} defined the $\UI(X;Y\backslash Z)$ to be the minimum information that $Y$ holds on $X$ given the marginal distributions of $(X,Y)$ and $(X,Z)$. Rauh et al.~in~\cite{rauh-bertschinger-olbrich-jost:ISIT:2014} proved that this decomposition is no more nonnegative in the multivariate case meaning that it cannot be extended to the multivariate case. In this paper, we are going to compute the optimization problem defined by Bertschinger et al.~to decompose the mutual information. But before defining their optimization problem, we point out that Harder et al.~in~\cite{harder2013bivariate} has also defined the decomposition based on projections in the probability simplex.  
%
